Sample-Efficient Reinforcement Learning with loglog(T) Switching Cost

We study the problem of reinforcement learning (RL) with low (policy) switching cost - a problem well-motivated by real-life RL applications in which deployments of new policies are costly and the number of policy updates must be low. In this paper, we propose a new algorithm based on stage-wise exploration and adaptive policy elimination that achieves a regret of $\widetilde{O}(\sqrt{H^4S^2AT})$ while requiring a switching cost of $O(HSA \log\log T)$. This is an exponential improvement over the best-known switching cost $O(H^2SA\log T)$ among existing methods with $\widetilde{O}(\mathrm{poly}(H,S,A)\sqrt{T})$ regret. In the above, $S,A$ denotes the number of states and actions in an $H$-horizon episodic Markov Decision Process model with unknown transitions, and $T$ is the number of steps. As a byproduct of our new techniques, we also derive a reward-free exploration algorithm with a switching cost of $O(HSA)$. Furthermore, we prove a pair of information-theoretical lower bounds which say that (1) Any no-regret algorithm must have a switching cost of $\Omega(HSA)$; (2) Any $\widetilde{O}(\sqrt{T})$ regret algorithm must incur a switching cost of $\Omega(HSA\log\log T)$. Both our algorithms are thus optimal in their switching costs.

==> sections/abstract.tex <==




 

==> sections/application.tex <==
% !TEX root = ../example_paper.tex


For the global switching cost of Algorithm~\ref{algo2}, we have the following conclusion.



We use a lemma from \cite{jin2020reward}. The proof of this lemma is dedicated and we include a proof for self-containedness in Appendix~\ref{appb}.

\begin{lemma}[Lemma C.2 in \cite{jin2020reward}]\label{lem13}
	Suppose $\widehat{\mathbb{P}}$ is the empirical transition matrix formed by sampling according to $\mu$ distribution for $N$ samples, $G$ can be any function from $\mathcal{S}$ to $[0,H]$, $\nu$ can be any function from $\mathcal{S}$ to $\mathcal{A}$, then with probability at least $1-\delta$, we have for any $h\in[H]$:
\begin{align*}	
&\max_{G:\mathcal{S}\rightarrow[0,H]}\max_{\nu:\mathcal{S}\rightarrow\mathcal{A}}\mathbb{E}_{\mu_{h}}|(\widehat{\mathbb{P}}_{h}-\mathbb{P}_{h})G(s,a)|^{2}\mathbb{I}\{a=\nu(s)\}\\ &\leq O(\frac{H^{2}S\log(HAN/\delta)}{N}).
\end{align*}
\end{lemma}

Recall that $\iota=\log(2HAK/\delta)$. We would like to state that for any policy and reward function, the value function under $\widetilde{P}$ and $\widehat{P}$ are close to each other. The proof of Lemma~\ref{lem14} is deferred to Appendix~\ref{appb}.
\begin{lemma}\label{lem14}
	Conditioned on the fact that $P^{int}$ is $\frac{1}{H}$-multiplicatively accurate to $\widetilde{P}$ (the case in Lemma~\ref{lem6}), with probability $1-\frac{T\delta}{2K}$, for any policy $\pi\in\phi$ and any reward function $r^{\prime}$, $$|V^{\pi}(r^{\prime},\widehat{P})-V^{\pi}(r^{\prime},\widetilde{P})|=O(\sqrt{\frac{H^{5}S^{2}A\iota}{T}}).$$
\end{lemma}







%\newpage

==> sections/simulation.tex <==
% !TEX root = ../example_paper.tex

Under non-Markov setting, the agent is allowed to use a mixture of deterministic policies. Our algorithms can be used under this setting with a natural modification. Recall that in Exploration (Algorithm~\ref{algo1}), for each layer $h$, we apply each $\pi_{h,s,a}$ ($(s,a)\in \mathcal{S}\times\mathcal{A}$) for the same number of episodes $\frac{T}{HSA}$. If we apply a mixture of all these $\pi_{h,s,a}$, which defined as $\pi_{h}$ such that $\pi_{h}=\pi_{h,s,a}$ with probability $\frac{1}{SA}$, then we can apply $\pi_{h}$ for $\frac{T}{H}$ episodes instead. The algorithm will have the same exploration effect with global switching cost only $H$. Using the same idea, in Evaluation (Algorithm~\ref{algo2}), we can apply $\pi_{random}$ that chooses each $\pi_{h,s,a}$ with probability $\frac{1}{HSA}$, $\forall\,(h,s,a)\in[H]\times \mathcal{S}\times\mathcal{A}$. Then the global switching cost for Algorithm~\ref{algo2} will be only $1$. Under a new schedule of Exploration and Evaluation, we have the following result.
\begin{theorem}\label{the6}
Under non-Markov setting, Algorithm~\ref{algo5} can achieve $\widetilde{O}(\sqrt{H^{4}S^{2}AT})$ regret while global switching cost is bounded by $2H+O(\log\log T)$.
\begin{remark}
We can see that under non-Markov setting, we can save a factor of $HSA$ for global switching cost.
\end{remark}
\end{theorem}
